A Hoare Logic for Domain Specification (Full Version)

Programs must be correct with respect to their application domain. Yet, the program specification and verification approaches so far only consider correctness in terms of computations. In this work, we present a two-tier Hoare Logic that integrates assertions for both implementation and domain. For domain specification, we use description logics and semantic lifting, a recently proposed approach to interpret a program as a knowledge graph. We present a calculus that uses translations between both kinds of assertions, thus separating the concerns in specification, but enabling the use of description logic in verification.

==> old.tex <==
\section{Introduction}
We investigate specification of programs that require to express constraints in terms of both the \emph{implementation} and the \emph{domain}. Such programs are critical in, for example, model-based engineering, where they are refined into controllers, or in Digital Twins where domain knowledge is needed in the simulation models.
While the implementation specification (IS) is well-explored in, e.g., Hoare logic-style verification, domain-specific specification (DSS) is an open challenge.
Domain-specific specification enables to involve domain experts in modeling by giving them a tool to express their constraints without 
exposing them to implementation details. Furthermore, this clear separation of concerns allows us to use different formalisms to reason about IS and DSS.

While this separation has a certain methodological elegance for specification, it poses a challenge to verification: program logics 
are explored mostly for assertion-expressions or incorporate expressions and other elements of the programs, such as variable names for frames.
Hoare logic heavily relies on this explicit inclusion or program elements in a expression-like term language through its substitution.
DSS, on the other hand, must be necessarily include all expression of the program, nor enable syntactical substitution.
\dg{Couldn't understand this sentence.}

Here, we investigate DSS in the context of \emph{semantically lifted programs}, program, whose states have a \emph{lifting} into a knowledge graph enriched with domain knowledge, which enables to interpret the program state in terms of the domain.
The specification is using only the notions and vocabulary of the lifted state, thus abstracting fully away from the implementation.
While we can refer to variables and their values, we cannot refer, or evaluate, more complex expressions.
The program itself is not lifted, so a program logic must operate in terms of the implementation language, but \emph{with respect to a lifted specification}.
We present weakest-precondition reasoning using a Hoare-logic for \emph{two-tier} specifications, that keeps track of the specification in terms of both implementation and domain, thus allowing to specify program behavior on two levels on abstraction.

We give a precise description on the connection between IS and DSS, and the elements required to set up the two-tier Hoare Logic.




\EK{how do invariants work?}

\EK{old and busted}

\begin{figure}

\begin{prooftree}
\AxiomC{$\phi_1 \rightarrow \phi_1'$}
\AxiomC{$\mathbf{C}\vdash \driple{\phi_1'}{\psi_1'} \statement \driple{\phi_2'}{\psi_2'}$}
\AxiomC{$\psi_1 \rightarrow \psi_1'$}
\LeftLabel{\rulename{strengthen}}
\TrinaryInfC{$\mathbf{C}\vdash \driple{\phi_1}{\psi_1} \statement \driple{\phi_2}{\psi_2}$}
\end{prooftree}

\EK{addmore}
    \caption{Basic Hoare calculus rules.}
    \label{fig:rules:core}
\end{figure}

The general rules for control-flow and other basix operations are given in Fig.~\ref{fig:rules:core}. The interesting rules are concerned with assignment, strengthening and moving information between the components of a lifted assertion.

Fig.~\ref{fig:rules:move} shows the rules concerned with manipulating lifted assertions.
We allow at any point to use $\abduct$ to get more information about the post-state, this is rule \rulename{generate-core}. A subtle point here is that this rule is \emph{non-deterministic} -- abduction can produce multiple explanations, and a strongest explanation is not guaranteed to exist (in particular if we there is no disjunction in the logic). This poses no challenges for soundness: once $\abduct$ has chosen one explanation for the post-condition, we must still prove that our pre-condition for the triple establishes it. Rule \rulename{lift-post} merely applies the lifting of specification, while \rulename{invert-post} applies its inverse. It has a side-condition that ensures that the lifting is indeed invertable here (because it must be an extension of $\liftdirect$). We note that the term generate by \rulename{generate-core} is guaranteed to satisfy this condition. Rules \rulename{invert-pre} and \rulename{list-pre} are analogous for preconditions. Note that abduction in the precondition is not sound and breaks the contract.

\begin{figure}
\begin{prooftree}
\AxiomC{$\mathbf{C}\vdash \driple{\phi_1}{\psi_1} s \driple{\phi_2}{\psi_2, \alpha(\psi_2 )}$}
\LeftLabel{\rulename{generate-core}}
\UnaryInfC{$\mathbf{C}\vdash \driple{\phi_1}{\psi_1} s \driple{\phi_2}{\psi_2}$}
\end{prooftree}

\begin{minipage}{0.6\textwidth}
\begin{prooftree}
\AxiomC{$\mathbf{C}\vdash \driple{\phi_1}{\psi_1} s \driple{\phi_2 \wedge \hat{\mu}^{-1}(\psi_2')}{\psi_2 , \psi_2'}$}
\LeftLabel{\rulename{invert-post}}
\RightLabel{$\mathsf{sig}(\psi_2') \subseteq \Sigma_\mathsf{dvar}$}
\UnaryInfC{$\mathbf{C}\vdash \driple{\phi_1}{\psi_1} s \driple{\phi_2}{\psi_2 , \psi_2'}$}
\end{prooftree}
\end{minipage}
\begin{minipage}{0.4\textwidth}
\begin{prooftree}
\AxiomC{$\mathbf{C}\vdash \driple{\phi_1}{\psi_1} s \driple{\phi_2}{\psi_2 , \hat\mu(\phi_2)}$}
\LeftLabel{\rulename{lift-post}}
\UnaryInfC{$\mathbf{C}\vdash \driple{\phi_1}{\psi_1} s \driple{\phi_2}{\psi_2}$}
\end{prooftree}
\end{minipage}

\begin{minipage}{0.6\textwidth}
\begin{prooftree}
\AxiomC{$\mathbf{C}\vdash \driple{\phi_1\wedge \hat{\mu}^{-1}(\psi_1')}{\psi_1} s \driple{\phi_2 }{\psi_2 , \psi_2'}$}
\LeftLabel{\rulename{invert-pre}}
\RightLabel{$\mathsf{sig}(\psi_2') \subseteq \Sigma_\mathsf{dvar}$}
\UnaryInfC{$\mathbf{C}\vdash \driple{\phi_1}{\psi_1} s \driple{\phi_2}{\psi_2 , \psi_2'}$}
\end{prooftree}
\end{minipage}
\begin{minipage}{0.4\textwidth}
\begin{prooftree}
\AxiomC{$\mathbf{C}\vdash \driple{\phi_1}{\psi_1, \hat\mu(\phi_1)} s \driple{\phi_2}{\psi_2}$}
\LeftLabel{\rulename{lift-pre}}
\UnaryInfC{$\mathbf{C}\vdash \driple{\phi_1}{\psi_1} s \driple{\phi_2}{\psi_2}$}
\end{prooftree}
\end{minipage}
    \caption{Rules to manipulate lifted assertions.}
    \label{fig:rules:move}
\end{figure}

Fig.~\ref{fig:rules:assign} shows the rules for assignment. We focus on the assignment to variables, rule \rulename{assign-rec} for records is analogous.
Rule \rulename{assign} performs the usual substitution on the state assertion. For the domain, the specification is \emph{removed}. The reason is that we do not know what effect the substitution has in the domain. Here we also remind that the domain logic is not only not closed under substitution -- it may not even contain the terms needed for substitution. Obviously, we must reconstruct the domain knowledge at this point using \rulename{list-pre}.

\begin{figure}
\begin{minipage}{0.42\textwidth}
\begin{prooftree}
\AxiomC{}
\LeftLabel{\rulename{assign}}
\UnaryInfC{$\mathbf{C}\vdash \driple{\phi_2[v \setminus e]}{\liftspec(\phi_2[v \setminus e])} v := e \driple{\phi_2}{\psi_2}$}
\end{prooftree}
\end{minipage}
\begin{minipage}{0.6\textwidth}
\begin{prooftree}
\AxiomC{}
\LeftLabel{\rulename{assign-rec}}
\UnaryInfC{$\mathbf{C}\vdash \driple{e \neq \mathtt{null} \wedge \phi_2[e.v \setminus e]}{\liftspec(e \neq \mathtt{null} \wedge \phi_2[e.v \setminus e])} e.v := e \driple{\phi_2}{\psi_2}$}
\end{prooftree}
\end{minipage}
    \caption{Rules for assignment}
    \label{fig:rules:assign}
\end{figure}

Let us prove the contract of $\mathtt{addDoors}$ with these rules.

To demonstrate the calculus, let us attempt to verify the contract for \texttt{addDoors}.
First, we derive information about the state, as expressed in the domain using \rulename{generate-core}. 
Using \rulename{strengthen-state} we pull this information into the program-specific part.
Let $\statement_\mathsf{door} = \mathtt{body.nrDoors~:=~doors;}$

\begin{prooftree}
\AxiomC{$A$}
\UnaryInfC{$
\driple{\mathtt{doors} = 2}{\mathtt{HasBody(c)}}
\statement_\mathsf{door}
\driple{\mathtt{body.doors} = 2}{\mathtt{HasTwoDoors(c)} \wedge \mathtt{value(body_nrDoors,2)}}
$}
\LeftLabel{\rulename{invert-post}}
\UnaryInfC{$
\driple{\mathtt{doors} = 2}{\mathtt{HasBody(c)}}
\statement_\mathsf{door}
\driple{\cdot}{\mathtt{HasTwoDoors(c)} \wedge \mathtt{value(body_nrDoors,2)}}
$}
\LeftLabel{\rulename{generate-core}}
\UnaryInfC{$
\driple{\mathtt{doors} = 2}{\mathtt{HasBody(c)}}
\statement_\mathsf{door}
\driple{\cdot}{\mathtt{HasTwoDoors(c)}}
$}
\end{prooftree}

Before we can apply our assignment rule, it remain to strengthen the precondition and transfer information between the two parts of the precondition.
From the derived information, using standard deduction we arrive at the following.

\begin{prooftree}
\AxiomC{$
\mathtt{HasBody(c)} \rightarrow \mathtt{NonNull(body)}
$}
\AxiomC{$
B
$}
\LeftLabel{\rulename{strengthen}}
\BinaryInfC{$
\driple{\mathtt{doors} = 2}{\mathtt{HasBody(c)}}
\statement_\mathsf{door}
\driple{\mathtt{body.doors} = 2}{\mathtt{HasTwoDoors(c)} \wedge \mathtt{value(body_nrDoors,2)}}
$}
\UnaryInfC{$A$}
\end{prooftree}

\begin{prooftree}
\AxiomC{$
$}
\LeftLabel{\rulename{assign-record}}
\UnaryInfC{$
\driple{\mathtt{doors} = 2 \wedge \mathtt{body \neq \mathtt{null}}}{\mathtt{HasBody(c) \wedge NonNull(body) \wedge value(body_nrDoors,2)}}
\statement_\mathsf{door}
\driple{\mathtt{body.doors} = 2}{\mathtt{HasTwoDoors(c)} \wedge \mathtt{value(body_nrDoors,2)}}
$}
\LeftLabel{\rulename{strengthen}}
\UnaryInfC{$
\driple{\mathtt{doors} = 2}{\mathtt{HasBody(c) \wedge NonNull(body) \wedge value(body_nrDoors,2)}}
\statement_\mathsf{door}
\driple{\mathtt{body.doors} = 2}{\mathtt{HasTwoDoors(c)} \wedge \mathtt{value(body_nrDoors,2)}}
$}
\LeftLabel{\rulename{lift-pre}}
\UnaryInfC{$
\driple{\mathtt{doors} = 2}{\mathtt{HasBody(c) \wedge NonNull(body)}}
\statement_\mathsf{door}
\driple{\mathtt{body.doors} = 2}{\mathtt{HasTwoDoors(c)} \wedge \mathtt{value(body_nrDoors,2)}}
$}
\UnaryInfC{$B$}
\end{prooftree}

This schema (generate core through abduction, invert lifting, perform substitution, lift specification) can be summarized in the following lemma.



==> prelim_old.tex <==
We give the basic definitions for the logic we use to describe the states of the implemented program directly, 
as well as definitions for description logics for domain specification.

\begin{definition}[States]
Let $V$ be the set of program variables and $D$ be the set of values.
Let $\state: V \rightarrow D$ be a state, i.e., a mapping from variables to values.
Let $\mathtt{S}$ be the set of all states.
\end{definition}

We require that the state and the domain logic share the notion of a signature, where a signature $\Sigma$ is a set of predicate and function symbols.
Our state logic is a predicate logic over program variable to express expressions. 
% Additionally, our state logic uses logical variables. Logical variables are bound by quantifiers to some value and managed by the variable assignment, while program variables are part of the state.

%
\begin{definition}[State Logic]
Let $\Sigma$ be a signature.
State formulas $\statephi$ are defined by the following grammar, where $v$ ranges over program variables, $p$ over predicate symbols from $\Sigma$, and $f$ over function symbols from $\Sigma$.
\[
\statephi ::= \statephi \wedge \statephi ~|~ \neg \statephi ~|~t \doteq t~|~ p(\overline{t}) 
\qquad\qquad t ::= v ~|~ x ~|~ f(\overline{t})
\]
We use the usual abbreviations such as $\vee$ and~$\rightarrow$.
The semantics of the state logic is completely standard and given in Fig.~\ref{fig:fol:sem}.
Let $\beta$ be a map from logical variables to values, $\sigma$ a state and $I$ a interpretation, i.e., a map from all symbols in~$\Sigma$ to predicates and functions.
\begin{figure}
\begin{align*}
    \sigma, \beta, I &\models \statephi_1 \wedge \statephi_2 \iff \sigma, \beta, I \models \statephi_1 \text{ and } \sigma, \beta, I \models \statephi_2 \\
    \sigma, \beta, I &\models \neg\statephi \iff \sigma, \beta, I \not\models \statephi\\% \sigma, \beta, I &\models \exists x.~\statephi \iff \sigma, \beta[x \mapsto d], I \models \statephi \text{ for some $d \in D$}  \\
    \sigma, \beta, I &\models t_! \doteq t_2 \iff \mathit{val}_{\sigma,\beta,I}(t_1) = \mathit{val}_{\sigma,\beta,I}(t_2)\\
    \sigma, \beta, I &\models p(t_1,\dots,t_n) \iff I(p)(\mathit{val}_{\sigma,\beta,I}(t_1),\dots, \mathit{val}_{\sigma,\beta,I}(t_n))\\ \\
    \mathit{val}_{\sigma,\beta,I}(v) &= \sigma(v) \qquad %\mathit{val}_{\sigma,\beta,I}(x) = \beta(x)\\
    \mathit{val}_{\sigma,\beta,I}(f(t_1,\dots,t_n)) = I(f)(\mathit{val}_{\sigma,\beta,I}(t_1),\dots, \mathit{val}_{\sigma,\beta,I}(t_n))
\end{align*}
    \caption{Semantics of the state logic.}
    \label{fig:fol:sem}
\end{figure}
\end{definition}

We define a simple description logic, $\mathcal{ACLO}(\mathsf{D})$, following mostly the semantics of Horrocks and Sattler~\cite{DBLP:conf/ijcai/HorrocksS01} for $\mathcal{SHON}(\mathsf{D})$, and its semantics. We stress that our approach is not relying on any particular property of this logic (or any description logic) except the presence of data types, and that we use it for the examples and envision description logics as the most suited formalism for domain specification in our framework.

\begin{definition}[Domain Logic]
The syntax of domain formulas $\liftphi$  is defined over atomic concepts $A$, abstract roles $R$, concrete roles $T$, nominals $o$ and data values~$d$.
\begin{align*}
    \liftphi ::=\>& C \sqsubseteq C ~|~ C(o) ~|~ R(o,o) ~|~ R(o,d)\\
    C ::=\>& \top ~|~ \bot ~|~ A ~|~ \neg C ~|~ C \sqcup C ~|~ C \sqcap C ~|~ \exists R.C ~|~ \forall R.C ~|~ \exists T.d ~|~ \forall T.d
\end{align*}
\end{definition}
Intuitively, concepts are unary predicates, roles are binary predicates, and nominals and data values are constant and literals. Semantically, a domain formula is evaluated with respect to a domain $\nabla$, a data domain $\nabla_\mathbf{D}$ and an interpretation~$\mathcal{I}$ that maps concepts, roles, nominals and data values into the domains. This is formally given in Fig.~\ref{fig:dl:sem}.
%
\begin{figure}[b]
\begin{align*}
    \mathit{val}_\mathcal{I}(\top) &= \nabla \qquad\quad~  \mathit{val}_\mathcal{I}(\bot) = \emptyset \\
    \mathit{val}_\mathcal{I}(A) &= \mathcal{I}(A) \qquad \mathit{val}_\mathcal{I}(\neg C) = \nabla \setminus \mathit{val}_\mathcal{I}(C) \\
    \mathit{val}_\mathcal{I}(C \sqcup D) &= \mathit{val}_\mathcal{I}(C) \cup \mathit{val}_\mathcal{I}(D) \\
    \mathit{val}_\mathcal{I}(C \sqcap D) &= \mathit{val}_\mathcal{I}(C) \cap \mathit{val}_\mathcal{I}(D) \\
    \mathit{val}_\mathcal{I}(\exists R.C) &= \{x \in \nabla ~|~ \exists y.~(x,y) \in \mathcal{I}(R) \wedge y \in \mathcal{I}(C)\} \\
    \mathit{val}_\mathcal{I}(\forall R.C) &= \{x \in \nabla ~|~ \forall y.~(x,y) \in \mathcal{I}(R) \wedge y \in \mathcal{I}(C)\}\\
    \mathit{val}_\mathcal{I}(\exists T.d) &= \{x \in \nabla_\mathbf{D} ~|~ \exists y.~(x,y) \in \mathcal{I}(T) \wedge y \in \mathcal{I}(T)\} \\
    \mathit{val}_\mathcal{I}(\forall T.d) &= \{x \in \nabla_\mathbf{D} ~|~ \forall y.~(x,y) \in \mathcal{I}(T) \wedge y \in \mathcal{I}(T)\}\\ \\
    \nabla, \nabla_\mathbf{D}, \mathcal{I} \models C \subseteq D &\iff \mathit{val}_\mathcal{I}(C) \subseteq \mathit{val}_\mathcal{I}(D)\\
    \nabla, \nabla_\mathbf{D}, \mathcal{I} \models C(o) &\iff \mathit{val}_\mathcal{I}(c) \in \mathit{val}_\mathcal{I}(C)\\
    \nabla, \nabla_\mathbf{D}, \mathcal{I} \models R(o,o') &\iff (\mathit{val}_\mathcal{I}(c),\mathit{val}_\mathcal{I}(o')) \in \mathit{val}_\mathcal{I}(R)\\
    \nabla, \nabla_\mathbf{D}, \mathcal{I} \models R(o,d) &\iff (\mathit{val}_\mathcal{I}(c),\mathit{val}_\mathcal{I}(d)) \in \mathit{val}_\mathcal{I}(R)
\end{align*}
    \caption{Semantics of the domain logic.}
    \label{fig:dl:sem}
\end{figure}

However, to ease the connection with the state logic, we consider first-order logic states as models for description logic formulas, as given in Fig.~\ref{fig:dl:fosem}.
\EK{We must talk about models $M$ here, because the lifting is defined on models. also entailment $\models_\knowledge$ and conservative extensions.}

\begin{figure}
    \centering
    \caption{First-order semantics of the domain logic.}
    \label{fig:dl:fosem}
\end{figure}
\EG{Explain that domain states are models.}

\EG{Explain $\knowledge$.}

